First measurement of the Q^2 distribution of X(3915) single-tag two-photon production

We report the first measurement of the $Q^2$ distribution of $X(3915)$ produced by single-tag two-photon interactions. The decay mode used is $X(3915) \rightarrow J/\psi\omega$. The covered $Q^2$ region is from 1.5 (GeV/$c$)$^2$ to 10.0 (GeV/$c$)$^2$. We observe $7.9\pm 3.1({\rm stat.})\pm 1.5({\rm syst.})$ events, where we expect $4.1\pm 0.7$ events based on the $Q^2=0$ result from the no-tag two-photon process, extrapolated to higher $Q^2$ region using the $c\bar{c}$ model of Schuler, Berends, and van Gulik. The shape of the distribution is also consistent with this model; we note that statistical uncertainties are large.

==> Makefile <==
FILE=j3pi_arxiv

all :
	pdflatex ${FILE}
	bibtex ${FILE}
	pdflatex ${FILE}
	pdflatex ${FILE}
	pdflatex ${FILE}

bib :
	bibtex ${FILE}

plot :
	qpdfview ${FILE}.pdf

clean :
	rm -f ${FILE}.log ${FILE}.aux ${FILE}.dvi ${FILE}.bbl ${FILE}.blg \
	${FILE}.out ${FILE}Notes.bib *.bak

